SOS-based Stability Verification for Saturated INDI Control of Hybrid-VTOL Aircraft Pitch Rate Dynamics

Incremental nonlinear dynamic inversion (INDI) is a prominent flight-control strategy valued for its robust disturbance rejection; however, its formal stability verification has traditionally been limited to linearized dynamical models. This paper presents a formal nonlinear stability certificate for a saturated INDI pitch-rate controller for an open-loop unstable hybrid vertical take-off and landing (VTOL) aircraft by representing the INDI controller via an equivalent recurrent equilibrium network (REN). By casting the saturated INDI architecture as a REN, the closed-loop dynamics are exactly mapped to an augmented state-feedback system. This structural equivalence enables the use of sum of squares (SOS) programming to synthesize a locally valid Lyapunov function without relying on conservative bounding approximations. The resulting certificate yields an inner estimate of the region of attraction (RoA) that explicitly accounts for actuator saturation, formally verifying the controller's stability in operating regimes where standard linear margins lose their validity.

==> ReLU_semialgebraic_set.tex <==
\begin{tikzpicture}
  \begin{axis}[
      width=4.5cm,
      height=2.5cm,
      scale only axis,
      axis lines=middle,
      xmin=-4.5, xmax=4.5,
      ymin=-1.5, ymax=3.5,
      xtick={-4,-3,...,4},
      ytick={-1,0,...,4},
      grid=major,
      grid style={gray!30},
      % Axis label font
      xlabel={$x$},
      % ylabel={$\mathrm{ReLU}(x)$},
      ylabel={$\color{blue} \mathrm{ReLU}(x)$},
      xlabel style={
        at={(axis cs:3.75,0.125)},
        anchor=south west,
        font=\footnotesize,
        % fill=white,
        % fill opacity=0.9,
        % inner sep=2pt
      },
      ylabel style={
        at={(axis cs:0.125,2.5)},
        anchor=south west,
        font=\footnotesize,
        fill=white,
        fill opacity=0.9,
        inner sep=2pt,
      },
      % Tick label font and background
      tick label style={
        font=\scriptsize,
        % fill=white,
        % fill opacity=0.9,
        % inner sep=1pt
      },
    ]

    \addplot [
      pattern=north east lines,
      pattern color=gray,
      draw=none,
      fill opacity=0.75,
    ] coordinates {
      (-4.5,0)
      (4.5,0)
      (4.5,-1.5)
      (-4.5,-1.5)
      (-4.5,0)
    };

    \addplot [
      fill=gray,
      fill opacity=0.25,   % Adjust opacity as you like
      draw=none,
    ] coordinates {
      (-4.5,0)
      (4.5,0)
      (4.5,-1.5)
      (-4.5,-1.5)
      (-4.5,0)
    };

    \addplot [
      pattern=north west lines,
      pattern color=gray,
      draw=none,
      fill opacity=0.75,
    ] coordinates {
      (-1.5,-1.5)
      (3.5,3.5)
      (4.5,3.5)
      (4.5,-1.5)
      (-1.5,-1.5)
    };

    \addplot [
      fill=gray,
      fill opacity=0.25,   % Adjust opacity as you like
      draw=none,
    ] coordinates {
      (-1.5,-1.5)
      (3.5,3.5)
      (4.5,3.5)
      (4.5,-1.5)
      (-1.5,-1.5)
    };

     \draw[-Latex, thick, black] (axis cs:-2.5,-0.5) -- (axis cs:-2.5,0.75) node[above, font=\footnotesize] {};

     % \draw[-Latex, thick, black] (axis cs:2.5,-0.5) -- (axis cs:2.5,0.5) {};

     % \draw[-Latex, thick, black] (axis cs:2.353,1.647) -- (axis cs:1.647,2.353) {};

     \draw[-Latex, thick, black] (axis cs:2.353,1.647) -- (axis cs:1.5,2.5) {};


     % \draw[-Latex, thick, black] (axis cs:-0.5,-0.5) -- (axis cs:-0.5,0.5) node[above, font=\footnotesize]

    \addplot [thick, gray, domain=-1.5:0] {x};

    % Plot ReLU function
    \addplot[very thick, blue] {max(0,x)};

    % Red dashed line y = x
    \addplot [
      red,
      very thick,
      dashed,
      dash pattern=on 2pt off 5pt,
      domain=-4.5:4.5,
      samples=2, % just two points needed for a straight line
    ] {x};
    
    % Red dashed line y = 0 (x-axis)
    \addplot [
      red,
      very thick,
      dashed,
      dash pattern=on 2pt off 5pt,
      domain=-4.5:4.5,
      samples=2,
    ] {0};

    \draw[black, thick] (rel axis cs:0,0) rectangle (rel axis cs:1,1);
  \end{axis}
\end{tikzpicture}

% \begin{tikzpicture}
%   \begin{axis}[
%       width=5cm,
%       height=3cm,
%       scale only axis,
%       axis lines=middle,
%       xmin=-4.5, xmax=4.5,
%       ymin=-1.5, ymax=3.5,
%       xtick={-4,-3,...,4},
%       ytick={-1,0,...,4},
%       grid=major,
%       grid style={gray!30},
%       % Axis label font
%       xlabel={$x$},
%       ylabel={$\mathrm{ReLU}(x)$},
%       xlabel style={
%         at={(axis cs:4,0.125)},
%         anchor=south west,
%         font=\footnotesize,
%         fill=white,
%         fill opacity=0.9,
%         inner sep=2pt
%       },
%       ylabel style={
%         at={(axis cs:0.125,3)},
%         anchor=south west,
%         font=\footnotesize,
%         fill=white,
%         fill opacity=0.9,
%         inner sep=2pt
%       },
%       % Tick label font and background
%       tick label style={
%         font=\footnotesize,
%         fill=white,
%         fill opacity=0.9,
%         inner sep=1pt
%       },
%     ]

%     \addplot[very thick, blue] {max(0,x)};
%   \end{axis}
% \end{tikzpicture}


% \begin{tikzpicture}
%   \begin{axis}[
%       % width=0.95\linewidth,
%       % % width=6cm,
%       % height=0.6\linewidth,
%       width = 5cm,
%       height = 2.5cm,
%       scale only axis,
%       % axis equal image,
%       axis lines=middle,
%       xmin=-4.5, xmax=4.5,
%       ymin=-1.5, ymax=3.5,
%       xtick={-4,-3,...,4},
%       ytick={-1,0,...,4},
%       grid=major,
%       grid style={gray!30},
%       xlabel={$x$},
%       ylabel={$f(x) = \text{ReLU}(x)$},
%       xlabel style={
%         at={(axis cs:4,0)},  % Position at rightmost x-tick
%         anchor=north west,
%         font=\footnotesize
%       },
%       ylabel style={
%         at={(axis cs:0,4)},  % Position at top y-tick
%         anchor=south west,
%         font=\footnotesize
%       },
%       tick label style={font=\footnotesize},
%       label style={font=\footnotesize},
%       domain=-5:5,
%       samples=200,
%     ]
%     \addplot[very thick, blue] {max(0,x)};
%   \end{axis}
% \end{tikzpicture}

% \begin{tikzpicture}
%   \begin{axis}[
%       width=0.95\linewidth,
%       height=0.6\linewidth,
%       axis lines=middle,
%       xlabel={$x$},
%       ylabel={$f(x) = \text{ReLU}(x)$},
%       xlabel style={at={(ticklabel* cs:1)}, anchor=north west, font=\small},
%       ylabel style={at={(ticklabel* cs:1)}, anchor=south east, font=\small},
%       xmin=-5, xmax=5,
%       ymin=-1.5, ymax=4.5,
%       xtick={-5,-4,...,5},
%       ytick={-1,0,...,4},
%       grid=both,
%       grid style={gray!30},
%       minor tick num=1,
%       tick label style={font=\small},
%       label style={font=\small},
%       domain=-5:5,
%       samples=200,
%     ]
%     \addplot[very thick, blue] {max(0,x)};
%   \end{axis}
% \end{tikzpicture}

% \begin{tikzpicture}
%   \begin{axis}[
%       width=\linewidth,
%       height=0.6\linewidth,
%       axis lines=middle,
%       xlabel={$x$},
%       ylabel={$f(x) = \text{ReLU}(x)$},
%       xmin=-5, xmax=5,
%       ymin=-1.5, ymax=4.5,
%       xtick={-5,-4,...,5},
%       ytick={-1,0,...,4},
%       grid=both,
%       grid style={gray!30},
%       minor tick num=1,
%       tick label style={font=\small},
%       label style={font=\small},
%       every axis x label/.style={at={(axis description cs:1.05,0)},anchor=west},
%       every axis y label/.style={at={(axis description cs:0,1.05)},anchor=south},
%       domain=-5:5,
%       samples=200,
%     ]
%     \addplot[very thick, blue] {max(0,x)};
%   \end{axis}
% \end{tikzpicture}
